Pangea: Monolithic Distributed Storage for Data Analytics

Storage and memory systems for modern data analytics are heavily layered, managing shared persistent data, cached data, and non-shared execution data in separate systems such as distributed file system like HDFS, in-memory file system like Alluxio and computation framework like Spark. Such layering introduces significant performance and management costs for copying data across layers redundantly and deciding proper resource allocation for all layers. In this paper we propose a single system called Pangea that can manage all data---both intermediate and long-lived data, and their buffer/caching, data placement optimization, and failure recovery---all in one monolithic storage system, without any layering. We present a detailed performance evaluation of Pangea and show that its performance compares favorably with several widely used layered systems such as Spark.

==> caseStudy.tex <==

\section{Case Study: Processing Complex Objects Using Pangea}
\label{sec:objectmodel}

In this section we describe a case study for processing complex and highly-nested objects using Pangea services.

In this particular implementation, to support high performance processing of complex and highly nested objects, all objects cached or stored in Pangea must be either a simple C++ object that doesn't contain virtual function call and pointers, or created using PC object model. 

PC object model~\cite{zou2017plinycompute} is a set of APIs for creating, deleting, and moving C++ objects for cluster computing.
   
An ordinary object in C++ or other languages, which contains virtual functions or pointers/references, can not be directly moved from memory to disk or vice versa,
can not be directly moved from one OS process to another OS process, and thus can not be moved from one cluster node to another cluster node.
After above moving, virtual function call and pointers will not work any more,  because all pointers, including VTable pointer that is used to dispatch virtual functions,  points to a
 memory address that is specific to only one OS process. As a result, an object must be serialized before it is to be moved away from the process where it is created; and must be deserialized into a new object instance before it is to be loaded into a new process.

C++ objects created with PC object model is different and can eliminate the (de)serialization overhead. 
\begin{enumerate}[leftmargin=*]
\item A PC object must be associated with and allocated in an allocation block, which is a piece of contiguous memory;
\item PC object model provides an alternative for C-style pointer, called \texttt{Handle}, which uses offsets rather than absolute memory addresses, so a PC object can be moved from process to process if it is moved together with its allocation block. Each creation of PC object through the \texttt{makeObject<T>(args...)} API returns a \texttt{Handle} that points to the created object~\cite{zou2017plinycompute}.
\end{enumerate}

A type of PC objects must be registered in form of shared library before being stored to Pangea. After registration, the type is associated with a unique type ID that is embeded in each PC object. Each storage or computation process maintains a hash map that maps the type ID to the valid VTable pointer address, for each PC object type met in this process. Supported by most compilers, the VTable pointer address of a C++ object can be obtained by creating an instance of this object using the registered shared library and then extracting the first eight bytes. Then, when a PC object is to be used (e.g. when derefencing a \texttt{Handle} or when invoking a \texttt{Handle}'s arrow operator and so on), the PC object's type ID will be extracted and used to look up the valid VTable pointer address in the hash map for fixing the outdated VTable pointer address only when necessary.


\vspace{5pt}
Pangea is designed to fully utilize the benefit of PC object model while alleviating its overhead.

\vspace{5pt}
Firstly, a Pangea page is used as allocation block for holding PC objects.

On each node, to write objects to a locality set in parallel, each thread in storage or computation process is associated with a PC allocator. Each thread pins a page in shared memory pool for that locality set, and passes the starting address of the page and page size to the PC allocator. Then all objects created using PC object model API in this thread are allocated in the allocation block. When the allocation block becomes full, the allocator will throw an exception. Depending on the purpose of the storage and computation thread, the exception will be caught with different processing:

\begin{itemize}[leftmargin=*]
\item \textbf{Persisting to Disk.} If the thread is writing objects to a \texttt{write-through} locality set (listed in the \texttt{durabilityType} category in Tab.~\ref{tab:attributes}), which requires all pages to be persisted to disk (for example, when a client dispatches objects to an input dataset, or when computation threads write objects as application output), a finished page is often written to disk. Under the hood, a page is appended to the flushing queue and one of the flushing threads will write the page to its underlying file instance and then unpin each written page from shared memory pool, so that the page is available for being evicted from memory whenever memory resources become insufficient. 

\item \textbf{Transimitting over Network.} if the thread is a computation thread for repartitioning objects across network for aggregation or join, a finished page is often compressed and sent to a remote node through Pangea's API. After the transmit is done, at the sender side, the page is unpinned; and at the receiver side, the received page is uncompressed and directly added to a new locality set created for storing shuffled data. As the repartitioned data is intermediate data and will not be reused, such data is often stored in a \texttt{write-back} locality set (also listed in the \texttt{durabilityType} category in Tab.~\ref{tab:attributes}), so that the pages will be cached in memory as long as possible, and will only be written back only when memory becomes insufficient.
\end{itemize}

\noindent
Both processing requires zero (de)serialization overhead when manipulating objects.

\vspace{5pt}
Secondly, a locality set stores a large number of objects having the same type, so that most of the VTable fixing overhead (e.g. loading the registered shared library to each storage or computation process on each node, and creating an object instance in each process for extracting the valid VTable pointer address), can be amortized to all objects stored in locality sets having the same type. The profiling results show that the rest of overhead (e.g. updating the VTable pointer for each object) is totally inlined and negligible.



